H3R: Hybrid Multi-view Correspondence for Generalizable 3D Reconstruction

Despite recent advances in feed-forward 3D Gaussian Splatting, generalizable 3D reconstruction remains challenging, particularly in multi-view correspondence modeling. Existing approaches face a fundamental trade-off: explicit methods achieve geometric precision but struggle with ambiguous regions, while implicit methods provide robustness but suffer from slow convergence. We present H3R, a hybrid framework that addresses this limitation by integrating volumetric latent fusion with attention-based feature aggregation. Our framework consists of two complementary components: an efficient latent volume that enforces geometric consistency through epipolar constraints, and a camera-aware Transformer that leverages Pl\"ucker coordinates for adaptive correspondence refinement. By integrating both paradigms, our approach enhances generalization while converging 2$\times$ faster than existing methods. Furthermore, we show that spatial-aligned foundation models (e.g., SD-VAE) substantially outperform semantic-aligned models (e.g., DINOv2), resolving the mismatch between semantic representations and spatial reconstruction requirements. Our method supports variable-number and high-resolution input views while demonstrating robust cross-dataset generalization. Extensive experiments show that our method achieves state-of-the-art performance across multiple benchmarks, with significant PSNR improvements of 0.59 dB, 1.06 dB, and 0.22 dB on the RealEstate10K, ACID, and DTU datasets, respectively. Code is available at https://github.com/JiaHeng-DLUT/H3R.

==> ICCV_2025_H3R/figures/encoder_performance.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/encoder_performance_fig.pdf}
    \caption{
        \textbf{Performance comparison of various visual foundation models as
            encoders.}
        SD-VAE~\cite{rombach2022high} achieves the best performance with the fewest parameters, demonstrating exceptional effectiveness and efficiency.
        See Appendix~\cref{tab:encoder_performance} for detailed results.
    }
    \label{fig:encoder_performance}
\end{figure*}

==> ICCV_2025_H3R/figures/framework.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/framework_fig.pdf}
    \caption{
        \textbf{Overview of our generalizable 3D reconstruction framework H3R.}
        Our method generates pixel-aligned Gaussians without per-scene optimization, achieving high-fidelity 3D reconstruction.
        The framework comprises five key stages: \textbf{(i) Visual encoding}: We employ a visual foundation model to extract rich latents from each context view, encoding appearance and structural information essential for 3D reconstruction.
        \textbf{(ii) Epipolar matching}: These latents are then aligned and aggregated into a coherent latent volume using epipolar geometric constraints, establishing spatial correspondences across views.
        \textbf{(iii) Camera embedding}: To further strengthen these correspondences, we incorporate camera parameters via Plücker coordinates and apply multi-view attention to refine the latents.
        \textbf{(iv) Gaussian decoding}: A lightweight CNN-based decoder subsequently transforms these refined latents into pixel-aligned Gaussians.
        \textbf{(v) Real-time rendering}: Finally, the generated Gaussian splats enable high-fidelity, real-time novel view synthesis.
    }
    \label{fig:framework}
    \vspace{-1em}
\end{figure*}

==> ICCV_2025_H3R/figures/high_resolution.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/high_resolution_fig.pdf}
    \caption{
        \textbf{Impact of input resolution on RealEstate10K.}
        Using 512$\times$512 inputs, our H3R-$\beta$ achieves more accurate geometry and photorealistic texture than recent methods, particularly for sharp edges and complex surfaces.
    }
    \label{fig:high_resolution}
\end{figure*}

==> ICCV_2025_H3R/figures/overlap.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/overlap_psnr.pdf}
    \end{subfigure}
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/overlap_ssim.pdf}
    \end{subfigure}
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/overlap_lpips.pdf}
    \end{subfigure}
    \caption{
        \textbf{Comparison with MVSplat~\cite{chen2024mvsplat} across varying overlaps on RealEstate10K.}
        Our method consistently outperforms MVSplat across all overlaps, with particularly significant improvements under low-overlap scenarios.
        See Appendix~\cref{tab:overlap} for detailed results.
    }
    \label{fig:overlap}
\end{figure*}

==> ICCV_2025_H3R/figures/performance_scaling.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/performance_scaling_psnr.pdf}
    \end{subfigure}
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/performance_scaling_ssim.pdf}
    \end{subfigure}
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{
            figures/performance_scaling_lpips.pdf
        }
    \end{subfigure}
    \caption{
        \textbf{Performance scaling during pre-training.}
        H3R exhibits power-law scaling on RealEstate10K, where performance improves linearly with the logarithm of training steps, similar to scaling patterns observed in large language models~\cite{kaplan2020scaling,touvron2023llama,hoffmann2022training}.
        PSNR shows no signs of saturation even at 1 million training steps, indicating potential for further improvement.
    }
    \label{fig:performance_scaling}
\end{figure*}

==> ICCV_2025_H3R/figures/radar.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/radar_fig.pdf}
    \caption{
        \textbf{Comparison with state-of-the-art generalizable 3D reconstruction methods.}
        Our method consistently outperforms existing approaches across three datasets, demonstrating superior reconstruction performance and cross-dataset generalization.
    }
    \label{fig:radar}
    \vspace{-1em}
\end{figure}

==> ICCV_2025_H3R/figures/re10k2acid_dtu.tex <==
\begin{figure*}[!tbp]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/re10k2acid.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/re10k2dtu.pdf}
    \end{subfigure}
    \caption{
        \textbf{Cross-dataset generalization from indoor RealEstate10K to outdoor ACID (left) and object-centric DTU (right).}
    }
    \label{fig:re10k2acid_dtu}
\end{figure*}

==> ICCV_2025_H3R/figures/re10k_acid.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/re10k.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/acid.pdf}
    \end{subfigure}
    \caption{
        \textbf{Qualitative results on RealEstate10K (left) and ACID (right).} \textbf{See Appendix~\cref{fig:target_pose,fig:view_scaling_visual,fig:high_resolution} for more visualizations.}
    }
    \label{fig:re10k_acid}
\end{figure*}

==> ICCV_2025_H3R/figures/target_pose.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/target_pose_fig.pdf}
    \caption{
        \textbf{Impact of target camera poses on RealEstate10K.}
        Our method (H3R-$\alpha$) leverages target camera poses to generate more complete and view-aligned Gaussian splats, improving geometric coherence while mitigating artifacts, particularly in unobserved regions.
    }
    \label{fig:target_pose}
\end{figure*}

==> ICCV_2025_H3R/figures/view_scaling.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/view_scaling_psnr.pdf}
        \label{fig:view_scaling_psnr}
    \end{subfigure}
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/view_scaling_ssim.pdf}
        \label{fig:view_scaling_ssim}
    \end{subfigure}
    \begin{subfigure}
        {0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/view_scaling_lpips.pdf}
        \label{fig:view_scaling_lpips}
    \end{subfigure}
    \vspace{-2em}
    \caption{
        \textbf{Comparison with MVSplat~\cite{chen2024mvsplat} across varying input
            views on RealEstate10K.}
        Our method outperforms MVSplat across all metrics and scales better with additional input views, while MVSplat's performance declines.
        See Appendix~\cref{tab:view_scaling} for detailed results.
    }
    \label{fig:view_scaling}
\end{figure*}

==> ICCV_2025_H3R/figures/view_scaling_visual.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/view_scaling_visual_fig.pdf}
    \caption{
        \textbf{Impact of the number of input views on RealEstate10K.}
        Increasing input views from two to eight enhances geometric completeness and visual fidelity, particularly for scene boundaries and specular surfaces.
    }
    \label{fig:view_scaling_visual}
\end{figure*}

==> ICCV_2025_H3R/preamble.tex <==
\usepackage{bm} % bold math symbols
\usepackage{booktabs} % better table rules (\toprule, \midrule, \bottomrule)
\usepackage{colortbl} % cell background colors (\cellcolor)
\usepackage{multirow, multicol, makecell} % row/column spans & flexible cell formatting
\usepackage{pifont} % % ✓ and ✗ symbols (\cmark, \xmark)
\usepackage[dvipsnames]{xcolor} % extra named colors
\usepackage{chngcntr} % adjust counter settings
\usepackage{nicematrix} % advanced table/matrix features
\usepackage{caption} % adjust caption spacing
\captionsetup{skip=5pt,belowskip=-5pt,position=bottom}
\usepackage{stfloats} % allow table* at bottom in two-column layout

\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

% colors
\definecolor{tabfirst}{rgb}{1,0.7,0.7}
\definecolor{tabsecond}{rgb}{1,0.85,0.7}
\definecolor{tabthird}{rgb}{1,1,0.7}
\definecolor{darkred}{rgb}{0.6,0.16,0.25}
\definecolor{heavygray}{gray}{0.90}
\newcommand{\gain}[1]{\textcolor{red}{#1}}
\newcommand{\diff}[1]{\footnotesize\textcolor{red}{\textbf{(#1)}}}


==> ICCV_2025_H3R/sec/0_abstract.tex <==
\begin{abstract}
    Despite recent advances in feed-forward 3D Gaussian Splatting, generalizable 3D reconstruction remains challenging, particularly in multi-view correspondence modeling.
    Existing approaches face a fundamental trade-off: explicit methods achieve geometric precision but struggle with ambiguous regions, while implicit methods provide robustness but suffer from slow convergence.
    We present H3R, a hybrid framework that addresses this limitation by integrating volumetric latent fusion with attention-based feature aggregation.
    Our framework consists of two complementary components: an efficient latent volume that enforces geometric consistency through epipolar constraints, and a camera-aware Transformer that leverages Plücker coordinates for adaptive correspondence refinement.
    By integrating both paradigms, our approach enhances generalization while converging 2$\times$ faster than existing methods.
    Furthermore, we show that spatial-aligned foundation models (e.g., SD-VAE) substantially outperform semantic-aligned models (e.g., DINOv2), resolving the mismatch between semantic representations and spatial reconstruction requirements.
    Our method supports variable-number and high-resolution input views while demonstrating robust cross-dataset generalization.
    Extensive experiments show that our method achieves state-of-the-art performance across multiple benchmarks, with significant PSNR improvements of 0.59 dB, 1.06 dB, and 0.22 dB on the RealEstate10K, ACID, and DTU datasets, respectively.
    Code is available at \url{https://github.com/JiaHeng-DLUT/H3R}.
\end{abstract}

==> ICCV_2025_H3R/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\input{figures/radar}

Generalizable 3D reconstruction~\cite{charatan2024pixelsplat,chen2024mvsplat,tang2024hisplat,zhang2024transplat,min2024epipolar,zhang2024gs,chen2024mvsplat360,wang2021ibrnet,wang2021neus,liu2024mvsgaussian,chan2023generative,xie2024lrm,hong2023lrm,trevithick2021grf,chen2021mvsnerf,liu2022neural,sajjadi2022scene,johari2022geonerf,cong2023enhancing,liu2023semantic,jiang2023leap,li2024gp,wang2024gs2} has attracted significant attention for its ability to recover 3D scenes without per-scene optimization.
Traditional Neural Radiance Fields (NeRF) require costly scene-specific training, limiting its practicality.
Recent advances~\cite{charatan2024pixelsplat,chen2024mvsplat,tang2024hisplat,zhang2024transplat,min2024epipolar,zhang2024gs,chen2024mvsplat360,liu2024mvsgaussian} shift toward feed-forward reconstruction methods that leverage efficient representations like 3D Gaussian Splatting (3DGS)~\cite{kerbl20233d,wang2024view}.
3DGS represents scenes as collections of 3D Gaussian primitives, bypassing the computationally intensive ray-marching of NeRF and enabling fast rasterization-based rendering.
pixelSplat~\cite{charatan2024pixelsplat} and MVSplat~\cite{chen2024mvsplat} predict pixel-aligned Gaussian primitives in a single forward pass, achieving high-quality reconstructions on real-world benchmarks.
Concurrently, Transformer-based approaches like eFreeSplat~\cite{min2024epipolar} and TranSplat~\cite{zhang2024transplat} improve cross-view correspondence through attention mechanisms, enhancing depth estimation from sparse inputs.
Despite substantial progress in reconstruction quality, significant challenges remain in achieving robust generalizable 3D reconstruction across diverse scenes.

The \textbf{first challenge} lies in \textit{the trade-off between explicit and implicit correspondence modeling.
}
Explicit methods~\cite{chen2024mvsplat,wang2024freesplat,liu2024mvsgaussian,fei2024pixelgaussian,tang2024hisplat,zheng2024gps} enforce geometric constraints through cost volumes, achieving high geometric precision but struggling when photometric consistency breaks down, \textit{e.g.}, under occlusions, textureless regions, specular highlights, or repetitive patterns~\cite{zhang2024transplat}.
In contrast, implicit methods~\cite{liu2023epipolar,johari2022geonerf,suhail2022generalizable,du2023learning,jin2024lvsm,hong2023lrm,xu2024grm,zhang2024gs} employ attention mechanisms to learn robust correspondences for ambiguous scenarios, but suffer from slow convergence~\cite{zhang2024gs,xu2024grm,tang2025lgm,hong2023lrm}.
Explicit methods deliver geometric precision but lack robustness, while implicit methods provide adaptability at the cost of efficiency.
Therefore, a principled integration of these paradigms is critical for robust and efficient multi-view correspondence modeling.

We present \textbf{H3R}, \textit{a hybrid network that integrates explicit and implicit correspondence modeling}.
It comprises two complementary components: volumetric latent fusion that enforces geometric consistency through epipolar constraints, and camera-aware Transformer that performs guided correspondence aggregation across viewpoints.
The volumetric module projects multi-view features into a discretized latent volume that explicitly captures geometric correspondences.
The Transformer leverages Plücker coordinates~\cite{royal1864philosophical} to perform geometry-informed attention, implicitly modeling cross-view correspondences.
This hybrid design achieves superior reconstruction quality while significantly improving training efficiency.

Beyond architectural design, we find that the choice of visual representation plays a critical role in determining correspondence quality.
This leads us to identify a \textbf{second key challenge}: \textit{the mismatch between the semantic nature of prevailing visual representations and the spatial fidelity required for 3D reconstruction}.
Recent methods~\cite{tang2024hisplat,charatan2024pixelsplat,chen2025lara,kulhanek2024wildgaussians,tang2025lgm,shen2025gamba,zhang2024geolrm,jena2025sparsplat,cao2024mvsformer++} typically rely on semantic-aligned models such as DINO~\cite{oquab2023dinov2,caron2021emerging}, which emphasize high-level semantic understanding through global image-level supervision.
However, this comes at the cost of pixel-level spatial fidelity, which is crucial for accurate 3D reconstruction.
In contrast, spatial-aligned models (such as MAE~\cite{he2022masked} and SD-VAE~\cite{rombach2022high}) preserve fine-grained local features and geometric structures through pixel-level reconstruction objectives, making them inherently more suitable for 3D reconstruction tasks that require precise cross-view correspondence.
Through systematic evaluation across diverse visual foundation models (\cref{fig:encoder_performance}), we demonstrate that \textit{spatial-aligned models consistently outperform semantic-aligned counterparts}.
Notably, SD-VAE achieves the optimal performance with superior parameter efficiency, while DINOv2 substantially underperforms despite widespread adoption.
These results provide strong evidence that spatial-aligned models are superior for generalizable 3D reconstruction.

Beyond these technical considerations, practical deployment presents challenges.
The \textbf{third challenge} stems from \textit{the variability of real-world inputs.
}
Existing methods assume controlled settings with fixed views and uniform quality, struggling with diverse real-world scenarios.
To address this deployment gap, we develop \textit{two specialized extensions} of our base H3R model.
H3R-$\alpha$ processes multiple context views through adaptive latent fusion, consistently improving reconstruction quality with additional views (\cref{fig:view_scaling}).
H3R-$\beta$ specializes in high-resolution reconstruction, delivering high-fidelity results with limited input views (\cref{tab:re10k_acid}).

Our key contributions are summarized as follows:
\begin{itemize}
    \item \textbf{Hybrid Multi-view Correspondence:}
          We introduce H3R, a hybrid framework that resolves the trade-off between explicit and implicit correspondence modeling.
          By unifying explicit volumetric fusion and implicit camera-aware Transformer, H3R achieves superior reconstruction quality across challenging scenes and converges 2$\times$ faster than state-of-the-art methods.
    \item \textbf{Spatial-aligned Visual Representation:}
          We systematically demonstrate that spatial-aligned visual representations significantly outperform conventional semantic-aligned features for high-fidelity 3D reconstruction.
          Notably, SD-VAE achieves the optimal performance with superior parameter efficiency, while DINOv2 substantially underperforms despite widespread adoption.
    \item \textbf{Comprehensive Performance Improvements:}
          We address three core challenges in generalizable 3D reconstruction, achieving state-of-the-art reconstruction quality (\cref{fig:radar}), strong generalization (\cref{tab:cross_dataset}), 2$\times$ faster convergence (\cref{tab:ablation}) and robust real-world adaptability (\cref{fig:view_scaling}).
          We demonstrate significant PSNR improvements of 0.59 dB, 1.06 dB, and 0.22 dB on RealEstate10K, ACID, and DTU datasets respectively.
\end{itemize}


==> ICCV_2025_H3R/sec/2_related_work.tex <==
\section{Related work}

\noindent\textbf{Generalizable 3D Gaussian Splatting.}
Recent 3DGS-based methods substantially improve the quality of generalizable 3D reconstruction.
Object-centric methods~\cite{szymanowicz2024splatter,chen2025lara,jianggaussianblock,xu2024grm,tang2025lgm,zhang2024gs,zou2024triplane}, trained on large-scale datasets~\cite{deitke2023objaverse,deitke2023objaversexl,qiu2024richdreamer}, achieve robust object reconstruction from sparse views and demonstrate strong generalization across diverse object categories.
In parallel, scene-level methods~\cite{charatan2024pixelsplat,chen2024mvsplat,zhang2024gs,zhang2024transplat,min2024epipolar,zheng2024gps} predict pixel-aligned Gaussian parameters to reconstruct unbounded scenes.
For example, pixelSplat~\cite{charatan2024pixelsplat} integrates epipolar Transformer with probabilistic depth sampling to resolve scale ambiguities.
GPS-Gaussian~\cite{zheng2024gps} and MVSplat~\cite{chen2024mvsplat} leverage cost volumes to improve geometric accuracy.
eFreeSplat~\cite{min2024epipolar} enforces depth consistency through iterative Gaussian alignment, and TranSplat~\cite{zhang2024transplat} refines Gaussian centers using monocular depth priors and depth-aware deformable matching.
Despite these advances, existing methods are often limited to sparse input views (1-4) and struggle in challenging real-world scenarios.
Therefore, we introduce a hybrid framework that accepts multi-view inputs, produces high-quality reconstructions, and exhibits strong generalization.

\noindent\textbf{Multi-view Stereo.}
Multi-view stereo (MVS) reconstructs 3D structure from a collection of calibrated 2D images~\cite{collins1996space} by exploiting either \textit{explicit} or \textit{implicit} multi-view correspondences.
Explicit cost volume methods~\cite{yao2018mvsnet,gu2020casmvsnet,ding2022transmvsnet,peng2022unimvsnet,xu2023unifying,xiong2023cl} build plane-sweep stereo volumes~\cite{collins1996space,yao2018mvsnet} to aggregate multi-view correspondences along epipolar lines, thus achieving efficient reconstruction.
However, they struggle in challenging scenarios where photometric consistency assumptions break down, such as occlusions, textureless surfaces, specular reflections, and repetitive patterns.
Conversely, attention-based methods~\cite{liu2023epipolar,johari2022geonerf,suhail2022generalizable,du2023learning,jin2024lvsm,hong2023lrm,xu2024grm,zhang2024gs} learn implicit correspondences via attention mechanisms, but often suffer from slow convergence~\cite{zhang2024gs,xu2024grm,tang2025lgm,hong2023lrm}.
To address these limitations, we propose a hybrid framework that combines explicit and implicit correspondences, leading to fast convergence and robust reconstruction across diverse scenes.

\noindent\textbf{Visual Foundation Models.}
Visual foundation models can be categorized by their supervision paradigm into \textit{semantic-aligned} and \textit{spatial-aligned} models.
Semantic-aligned models focus on global semantic understanding through image-level supervision.
While effective at capturing high-level holistic representations, these models often sacrifice spatial fidelity and visual details.
Representative examples include DeiT III~\cite{touvron2022deit} for image classification and CLIP~\cite{radford2021learning} for vision-language alignment.
In contrast, spatial-aligned models learn explicit spatial structures and fine-grained visual cues through pixel-aligned supervision.
Examples include Depth Anything~\cite{yang2024depth,yang2024depthv2} for depth estimation, SAM~\cite{kirillov2023segment,ravi2024sam} for semantic segmentation, DUSt3R~\cite{wang2024dust3r} and MASt3R~\cite{leroy2025grounding} for 3D point regression and matching, as well as MAE~\cite{he2022masked} and SD-VAE~\cite{rombach2022high} for image reconstruction.
Our experiments demonstrate that spatial-aligned backbones consistently outperform semantic-aligned counterparts, underscoring the importance of spatial-aligned supervision for generalizable 3D reconstruction.


==> ICCV_2025_H3R/sec/3_method.tex <==
\section{Method}

We propose H3R (\cref{fig:framework}), a hybrid multi-view correspondence framework for generalizable 3D reconstruction.
H3R combines volumetric latent fusion with a camera-aware Transformer, achieving superior rendering quality and accelerated convergence.
To handle varying inputs in practical 3D reconstruction scenarios, we develop two extensions of our base model.
H3R-$\alpha$ handles multiple context views and integrates target view poses to ensure comprehensive scene coverage, while H3R-$\beta$ specializes in high-resolution reconstruction and delivers high-quality results even with few input views.
We present the base H3R model in~\cref{sec:sparse_view_reconstruction} and detail the multi-view extension H3R-$\alpha$ in~\cref{sec:multiview_reconstruction}.

\subsection{Sparse-view Reconstruction}
\label{sec:sparse_view_reconstruction}

Given $N$ sparse context images $\{I_{i} \in \mathbb{R}^{H \times W \times 3}\}_{i=1}^{N}$, we first employ a visual foundation model $\mathcal{E}$ to independently encode each image $I_{i}$:
\begin{equation}
    \bm{x}_{i} = \mathcal{E}(I_{i}) \in \mathbb{R}^{h \times w \times c}.
\end{equation}
The core challenge lies in effectively fusing these per-view features $\{\bm{x}_i\}_{i=1}^N$ to generate a unified 3D Gaussian representation of the scene:
\begin{equation}
    f \colon \{\bm{x}_{i}\}_{i=1}^{N} \to \{\bm{G}_{j}\}_{j=1}^{N \times H \times W \times K},
\end{equation}
where $K$ represents the number of Gaussians per pixel.
We introduce two complementary modules designed to model cross-view relationships: volumetric latent fusion and camera-aware Transformer.

\input{figures/framework}

\noindent\textbf{Volumetric Latent Fusion.}
We construct latent volumes using epipolar geometry to capture cross-view correspondences.
Following plane-sweep stereo~\cite{collins1996space,yao2018mvsnet,im2019dpsnet,xu2023unifying}, we sample depth planes and warp neighboring view latents into the reference coordinate system.
Within the near and far depth bounds, we uniformly sample $d$ depth planes $\{\bm{D}^{k}\}_{k=1}^{d}$ in inverse depth space.
For each reference view $i$, we warp the latent $\bm{x}_{j}$ from neighboring view $j$ onto these depth planes via differentiable homography~\cite{yao2018mvsnet}:
\begin{equation}
    \bm{x}_{j \to i}^{k} = \text{Warp}(\bm{x}_{j}, \mathbf{P}_{i \to j}, \bm{D}^{k}) \in \mathbb{R}^{h \times w \times c},
\end{equation}
where $\mathbf{P}_{i \to j}$ denotes the relative camera projection from view $i$ to $j$.
We then concatenate the warped latents from all depth planes to construct the latent volume $\bm{x}_{j \to i}$:
\begin{equation}
    \bm{x}_{j \to i} = \left[\bm{x}_{j \to i}^{1}, \bm{x}_{j \to i}^{2}, \dots, \bm{x}_{j \to i}^{d}\right] \in \mathbb{R}^{h \times w \times d \times c},
\end{equation}
where $\left[\cdot\right]$ denotes concatenation along the depth dimension.

We evaluate three strategies for latent volume construction: \textit{correlation-based}, \textit{difference-based}, and \textit{cost-free}.
The \textit{correlation-based} approach, widely adopted in multi-view stereo~\cite{yao2018mvsnet}, measures feature similarity using the scaled dot product between reference features $\bm{x}_{i}$ and warped source features $\bm{x}_{j \to i}$:
\begin{equation}
    \bm{x}_{j \to i}^{\prime} = \frac{\bm{x}_{i} \cdot \bm{x}_{j \to i}}{\sqrt{c}} \in \mathbb{R}^{h \times w \times d},
\end{equation}
where $\bm{x}_{j \to i}^{\prime}$ represents the constructed latent volume.
This formulation produces distinct peaks at correct correspondences, particularly in texture-rich regions.
The \textit{difference-based} approach constructs the volume by concatenating element-wise feature differences across all $d$ depth planes:
\begin{equation}
    \bm{x}_{j \to i}^{\prime} = \bm{x}_{j \to i} - \bm{x}_{i} \in \mathbb{R}^{h \times w \times (d \times c)}.
\end{equation}
This strategy excels at localizing correspondences along sharp edges where feature disparities are most salient.
The cost-free approach forgoes explicit similarity metrics, directly concatenating warped features across depth planes:
\begin{equation}
    \bm{x}_{j \to i}^{\prime} = \bm{x}_{j \to i} \in \mathbb{R}^{h \times w \times (d \times c)}.
\end{equation}
This design preserves the complete feature representations, allowing subsequent layers to learn task-specific matching functions.
Our experiments (\cref{tab:cost_function}) demonstrate that the cost-free strategy achieves superior cross-dataset generalization compared to handcrafted methods.

To integrate multi-view information, we fuse original latent $\bm{x}_{i}$ with latent volume $\bm{x}_{i}^{\prime}$ through linear projections:
\begin{equation}
    \bm{z}_{i} = \mathrm{Linear}_{1}\left(\bm{x}_{i}\right) + \mathrm{Linear}_{2}\left(\bm{x}_{j \to i}^{\prime}\right) \in \mathbb{R}^{h \times w \times c^{\prime}},
\end{equation}
where $\mathrm{Linear}_{1}\colon \mathbb{R}^{c}\to \mathbb{R}^{c^{\prime}}$ and $\mathrm{Linear}_{2}\colon \mathbb{R}^{d \times c}\to \mathbb{R}^{c^{\prime}}$ project the latents into a shared $c^{\prime}$-dimensional space.

\noindent\textbf{Camera-aware Transformer.}
Camera parameters provide essential geometric constraints for 3D scene understanding, reconstruction, and reasoning~\cite{xu2023dmv3d,hong2023lrm,shi2023mvdream,liu2023zero}.
Pixel-aligned camera rays encode rich geometric priors that vary across spatial locations and viewpoints.
We leverage this information using Plücker ray coordinates~\cite{royal1864philosophical,xu2023dmv3d,zhang2024gs,tang2025lgm,xu2024grm}:
\begin{equation}
    \bm{r}_{i}=[\boldsymbol{o}_{i} \otimes \boldsymbol{d}_{i}, \boldsymbol{d}_{i}] \in \mathbb{R}^{h \times w \times 6},
\end{equation}
where $\boldsymbol{o}_{i}$ and $\boldsymbol{d}_{i}$ denote the origin and direction of each pixel ray for view $i$, and $\otimes$ represents cross product.

The visual tokens $\{\bm{z}_{i}\}_{i=1}^{N}$ and Plücker coordinates $\{\bm{r}_{i}\}_{i=1}^{N}$ from all input views are flattened and concatenated into 1D sequences $\bm{z} \in \mathbb{R}^{(N \times h \times w) \times c^{\prime}}$ and $\bm{r} \in \mathbb{R}^{(N \times h \times w) \times 6}$.
The Plücker coordinates are embedded and fused with visual tokens to enable camera conditioning.
Self-attention layers implicitly strengthen multi-view correlations, followed by a feed-forward network (FFN).
The process is formalized as:
\begin{equation}
    \begin{aligned}
        \bm{z} & = \bm{z} + \text{PosEmb}(\bm{r}),                      \\
        \bm{z} & = \bm{z} + \text{Attention}(\text{LayerNorm}(\bm{z})), \\
        \bm{z} & = \bm{z} + \text{FFN}(\text{LayerNorm}(\bm{z})).
    \end{aligned}
\end{equation}
Here, $\text{PosEmb}\colon \mathbb{R}^{6}\to \mathbb{R}^{c^{\prime}}$ maps Plücker coordinates to the feature dimension.

\noindent
\textbf{Gaussian Decoding.}
After processing through the camera-aware Transformer, we upsample the fused multi-view latents to the original input resolution and decode them into Gaussian parameters using a hierarchical CNN decoder $\mathcal{D}$:
\begin{equation}
    \bm{G} = \mathcal{D}(\bm{z}) \in \mathbb{R}^{N \times H \times W \times K}.
\end{equation}
The decoder $\mathcal{D}$ employs sequential upsampling ResBlocks~\cite{he2016deep}.
Following~\cite{zhang2024gs}, Gaussian primitives are parameterized by 3-channel RGB, 3-channel scale, 4-channel rotation quaternion, 1-channel opacity, and 1-channel ray distance.
For rendering, Gaussian center positions are derived from ray distances and camera parameters.
See Appendix~\cref{sec:gaussian_parameterization} for more details.

\noindent
\textbf{Training Loss.}
We employ mean-squared error ($\text{MSE}$) and learned perceptual image patch similarity ($\text{LPIPS}$)~\cite{zhang2018unreasonable} losses to supervise novel view synthesis, following~\cite{charatan2024pixelsplat,tang2024hisplat,chen2024mvsplat,zhang2024transplat,hong2023lrm,tang2025lgm,xu2024grm,zhang2024gs}.
We also incorporate mean-absolute-error ($\text{MAE}$) loss on image gradients to enhance photometric consistency.
The overall training objective is defined as:
\begin{equation}
    \label{eq:loss}
    \mathcal{L}_{\mathcal{D}} = \text{MSE}(I, \hat{I}) + \lambda \cdot \text{LPIPS}(I, \hat{I}) + \text{MAE}(\nabla I, \nabla \hat{I}),
\end{equation}
where $I$ and $\hat{I}$ denote the ground truth and rendered images, respectively, $\nabla$ is the gradient operator, and $\lambda = 0.05$ balances the $\text{LPIPS}$ loss.

\subsection{Multi-view Reconstruction}
\label{sec:multiview_reconstruction}

\noindent
\textbf{Handling Variable Input Views.}
To accommodate varying numbers of input views in real-world 3D reconstruction scenarios, we train our model on diverse view conditions and incorporate target view camera poses into the Gaussian generation process.
For multiple context views, we compute pixel-wise average of the warped latents during volumetric fusion, enabling adaptive input handling:
\begin{equation}
    \bm{x}_{i}^{\prime} = \frac{1}{N-1}\sum_{j \neq i}\bm{x}_{j\to i}^{\prime},
\end{equation}
where $\bm{x}_{i}^{\prime}$ denotes the fused latent volume for view $i$.
Our camera-aware Transformer architecture inherently supports dynamic input view counts.
As shown in~\cref{fig:view_scaling}, reconstruction quality consistently improves with increased views, demonstrating adaptability across varying input views.

\noindent
\textbf{Target View Integration.}
Existing generalizable 3DGS methods do not explicitly generate Gaussians for target views, limiting comprehensive scene reconstruction.
We address this limitation by incorporating target view camera poses (\textit{without corresponding images}) to generate pixel-aligned Gaussians for target views.
We use zero tensors for target view visual features while computing valid Plücker coordinates from their camera poses, feeding both into the Transformer.
This facilitates information exchange between context and target poses, enhancing Gaussian generation for complete view coverage.
A challenge is that without an explicit supervision, the model tends to ignore the target pose information during training.
To address this, we introduce an auxiliary reconstruction head that predicts target images from final-layer features, supervised by~\cref{eq:loss}.
This ensures target-view Gaussians actively participate in rendering, achieving comprehensive scene coverage.
Qualitative results are shown in Appendix~\cref{fig:target_pose}.


==> ICCV_2025_H3R/sec/4_experiments.tex <==
\section{Experiments}

\subsection{Main Results}

\noindent\textbf{Setup.}
H3R is pre-trained using two context views at a 256$\times$256 resolution.
We subsequently fine-tune two variants from this base model: 1) H3R-$\alpha$ supports 2-8 input views at the 256$\times$256 resolution and 2) H3R-$\beta$ accepts two context views at a higher 512$\times$512 resolution.
H3R-$\alpha$ also accepts target camera poses as input to generate Gaussians with comprehensive view coverage, which substantially improves rendering quality in unobserved regions.
See Appendix~\cref{sec:implementation_details} for more details.

\input{tables/re10k_acid}

\noindent\textbf{Two-view Novel View Synthesis.}
We evaluate our approach against state-of-the-art methods on two challenging datasets: RealEstate10K~\cite{zhou2018stereo} and ACID~\cite{liu2021infinite}, as presented in~\cref{tab:re10k_acid}.
On RealEstate10K, H3R outperforms TranSplat~\cite{zhang2024transplat} by a significant margin \gain{(+0.91 PSNR, +0.016 SSIM, and -0.011 LPIPS)}.
On ACID, our method achieves a PSNR of 28.29 and SSIM of 0.846, surpassing both pixelSplat~\cite{charatan2024pixelsplat} and MVSplat~\cite{chen2024mvsplat}.
The quantitative results, along with qualitative comparisons in~\cref{fig:re10k_acid}, demonstrate our method's effectiveness in producing high-fidelity novel views from sparse inputs.

\input{figures/re10k_acid}
\input{figures/view_scaling}

Our approach exhibits versatility through two specialized variants, each tailored for distinct input conditions.
H3R-$\alpha$ leverages target camera poses to generate Gaussians with comprehensive view coverage, achieving consistent improvements over the base H3R model (\gain{+0.19 and +0.15 PSNR} on RealEstate10K and ACID, respectively).
H3R-$\beta$ exploits higher-resolution inputs for enhanced detail capture, achieving superior rendering quality (\gain{+0.43 and +0.42 PSNR}).
These results demonstrate our approach's versatility across diverse input conditions, advancing state-of-the-art in generalizable novel view synthesis and highlighting potential for real-world deployment.

\noindent\textbf{Multi-view Novel View Synthesis.}
\cref{fig:view_scaling} compares the performance scaling trends of H3R-$\alpha$ with MVSplat~\cite{chen2024mvsplat} across varying number of input views on RealEstate10K.
H3R-$\alpha$ consistently improves with additional views, achieving \gain{+2.78 PSNR and -0.035 LPIPS} gains when scaling from 2 to 8 views.
In contrast, MVSplat~\cite{chen2024mvsplat} shows performance degradation (\gain{-6.01 PSNR}) in perceptual quality (\gain{+0.085 LPIPS}).
At 8 views, the performance gap reaches \gain{+9.89 PSNR and -0.134 LPIPS}.
The monotonic improvement across all metrics demonstrates H3R-$\alpha$'s superior adaptability for practical multi-view reconstruction scenarios.

\noindent\textbf{Cross-dataset Generalization.}
We evaluate cross-dataset generalization by training on RealEstate10K (indoor) and performing zero-shot evaluation on ACID (outdoor) and DTU (object-centric).
As shown in~\cref{tab:cross_dataset}, our approach consistently outperforms existing methods across both datasets.
Compared to TranSplat~\cite{zhang2024transplat}, H3R achieves substantial improvements of \gain{+0.62 PSNR, +0.012 SSIM, and -0.004 LPIPS} on ACID, and \gain{+0.22 PSNR, +0.062 SSIM, and -0.021 LPIPS} on DTU.
~\cref{fig:re10k2acid_dtu} demonstrates that our method produces high-fidelity outputs while baselines suffer from artifacts.
Our model variants H3R-$\alpha$ and H3R-$\beta$ further enhance performance, demonstrating robust generalization across diverse scene types.

\noindent\textbf{Robustness to varying overlaps.}
We partition the RealEstate10K dataset into overlap-based subsets to evaluate our model's robustness.
As illustrated in~\cref{fig:overlap}, our approach consistently outperforms MVSplat~\cite{chen2024mvsplat} across all overlap ranges, especially under low-overlap scenarios.
More specifically, our method achieves substantial gains of \gain{+1.72 PSNR, +0.036 SSIM, and -0.024 LPIPS} under the lowest overlap condition.
The robust performance stems from our integration of explicit volumetric latent fusion with implicit camera-aware Transformer, which effectively establishes strong cross-view relationships even when epipolar priors become insufficient.

\input{tables/cross_dataset}
\input{figures/re10k2acid_dtu}
\input{figures/overlap}
\input{figures/encoder_performance}

\subsection{Ablation Studies}

\noindent\textbf{Visual Encoder.}
We first evaluate various visual foundation models as 3D reconstruction encoders, spanning diverse training objectives, architectures, and scales (see Appendix~\cref{tab:encoder_type}).
As shown in~\cref{fig:encoder_performance}, models trained with pixel-aligned supervision (SD-VAE~\cite{rombach2022high}, MAE~\cite{he2022masked}, MAsT3R~\cite{leroy2025grounding}) systematically outperform those using semantic-aligned supervision (CLIP~\cite{radford2021learning}, DeiT-III~\cite{touvron2022deit}).
SD-VAE~\cite{rombach2022high} achieves optimal performance with superior parameter efficiency while DINOv2~\cite{oquab2023dinov2} substantially underperforms despite its widespread adoption.
This disparity highlights the limitations of semantic-oriented pre-training, which compromises fine-grained spatial information essential for precise geometry and appearance reconstruction.
Consequently, we adopt SD-VAE as our default encoder.

\noindent\textbf{Volumetric Latent Fusion.}
Our latent volume aggregates multi-view correspondences into a unified 3D representation, enabling robust view synthesis across diverse scenes.
As shown in~\cref{tab:plucker_latent}, this component achieves significant gains on RealEstate10K (\gain{+3.99 PSNR, +0.120 SSIM, -0.078 LPIPS}) and demonstrates strong zero-shot generalization: \gain{+4.15 PSNR} on ACID and \gain{+4.98 PSNR} on DTU.
When combined with Plücker coordinates, the latent volume contributes \gain{+3.55 PSNR} on DTU.
These results confirm that volumetric latent fusion effectively learns multi-view correspondences, enhancing reconstruction quality and cross-dataset generalization.

\noindent\textbf{Plücker Coordinates.}
Plücker coordinates provide a compact 6D parameterization of 3D rays, jointly encoding camera origin and viewing direction.
As shown in~\cref{tab:plucker_latent}, incorporating Plücker coordinates yields significant gains on RealEstate10K (\gain{+3.94 PSNR, +0.120 SSIM, -0.077 LPIPS}) and generalizes to unseen datasets: \gain{+3.92 PSNR} on ACID and \gain{+1.41 PSNR} on DTU.
While PSNR improvements become less pronounced when combined with latent volume, which already encodes positional information, Plücker coordinates still enhance perceptual quality on DTU (\gain{+0.025 SSIM, -0.007 LPIPS}).
These results demonstrate that geometric positional encoding complements volumetric correspondences, contributing to reconstruction quality and cross-dataset generalization.

\noindent\textbf{Cost Strategy.}
~\cref{tab:cost_function} evaluates different cost strategies for volumetric latent fusion.
While the difference-based cost computation achieves marginally higher performance on RealEstate10K and ACID, the cost-free approach performs best on the DTU benchmark with \gain{+0.011 SSIM and -0.007 LPIPS} improvements.
These results demonstrate superior generalization across diverse datasets, whereas explicit cost functions exhibit dataset-specific biases.
We adopt the cost-free approach as our default.

\noindent\textbf{Camera-aware Transformer.}
The camera-aware Transformer is essential for ensuring multi-view consistency in novel view synthesis.
As shown in~\cref{tab:ablation}, its removal leads to substantial performance degradation (\gain{-1.07 PSNR, -0.022 SSIM, +0.019 LPIPS}), underscoring its critical role in capturing cross-view relationships.
By incorporating viewpoint-specific information, this module enables the network to maintain geometric coherence across different camera poses, effectively handling occlusions and preserving 3D structural consistency in complex scenes.

\noindent\textbf{Gaussian Decoder.}
The hierarchical Gaussian decoder is essential to the reconstruction pipeline.
As shown in~\cref{tab:ablation}, its inclusion provides a substantial performance improvement (\gain{+2.47 PSNR, +0.072 SSIM, -0.080 LPIPS}), revealing that the progressive upsampling strategy is fundamental to accurate Gaussian parameter prediction.
This hierarchical design decomposes the complex prediction task into progressive refinement stages, facilitating both training stability and multi-scale feature propagation.

\noindent\textbf{Pixel Gradient Loss.}
The pixel gradient loss provides meaningful improvements in reconstruction quality.
As shown in~\cref{tab:ablation}, removing it degrades performance (\gain{-0.12 PSNR, -0.007 SSIM}).
This loss targets high-frequency details and local textures that standard reconstruction losses often overlook, helping preserve fine-grained visual quality.

\noindent\textbf{Convergence Speed.}
Our method demonstrates significant training efficiency.
As shown in~\cref{tab:ablation}, it achieves comparable performance to TranSplat~\cite{zhang2024transplat} in half the training steps (150k vs 300k).
This 2$\times$ speedup stems from the synergy between our latent volume for multi-view fusion, camera-aware Transformer for adaptive correspondence modeling, and hierarchical decoder for progressive refinement.

\input{tables/plucker_latent}
\input{tables/cost_function}
\input{tables/ablation}

==> ICCV_2025_H3R/sec/5_conclusion.tex <==
\section{Conclusion}

We introduced H3R, a hybrid framework that advances generalizable 3D reconstruction by addressing three fundamental challenges: the trade-off in multi-view correspondence modeling, the choice of visual representation and the variability of real-world inputs.
H3R synergistically combines the geometric precision of explicit constraints with the robustness of implicit attention-based aggregation.
By integrating a cost-free latent volume with a camera-aware Transformer, our model achieves both geometric precision and robust correspondence, converging $2\times$ faster than prior art.
Furthermore, we identified a critical mismatch between feature representation and reconstruction fidelity.
Our systematic analysis reveals that spatial-aligned foundation models (\textit{e.g.}, SD-VAE) significantly outperform widely adopted semantic-aligned models like DINOv2.
This provides a crucial insight for future work: prioritizing spatial fidelity over semantic abstraction is key to achieving high-fidelity 3D reconstruction.
Experimental results confirm our method's efficacy, demonstrating consistent improvements across multiple benchmarks and robust cross-dataset generalization while supporting variable-number or high-resolution input views.
H3R not only delivers superior performance but also provides foundational principles for designing more efficient and robust reconstruction systems.


==> ICCV_2025_H3R/sec/6_acknowledgments.tex <==
\clearpage
\section{Acknowledgments}
This work is partially supported by the National Science and Technology Major Project (Grant No.
2022ZD0117802), the Fundamental Research Funds for the Central Universities (Grant No. 226-2025-00055), and the Earth System Big Data Platform of the School of Earth Sciences, Zhejiang University.
This research is also supported by the Agency for Science, Technology and Research (A*STAR) under its MTC Programmatic Funds (Grant No.
M23L7b0021).


==> ICCV_2025_H3R/tables/ablation.tex <==
\begin{table}[!tbp]
    \centering
    \setlength{\tabcolsep}{2pt}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{c|c|ccc}
            \toprule
            \textbf{Step}         & \textbf{Design}                      & \textbf{PSNR$\uparrow$}               & \textbf{SSIM$\uparrow$}               & \textbf{LPIPS$\downarrow$}   \\
            \midrule
            \multirow{5}{*}{150k} & \cellcolor{heavygray}{Full}          & \cellcolor{heavygray}{\textbf{26.68}} & \cellcolor{heavygray}{\textbf{0.875}} & \cellcolor{heavygray}{0.126} \\
                                  & w/o camera-aware Transformer         & 25.61                                 & 0.853                                 & 0.145                        \\
                                  & w/o Gaussian decoder                 & 24.21                                 & 0.803                                 & 0.206                        \\
                                  & w/o pixel gradient loss              & 26.56                                 & 0.868                                 & \textbf{0.125}               \\
            \midrule
            \multirow{3}{*}{300k} & MVSplat~\cite{chen2024mvsplat}       & 26.39                                 & 0.869                                 & 0.128                        \\
                                  & eFreeSplat~\cite{min2024epipolar}    & 26.45                                 & 0.865                                 & 0.126                        \\
                                  & TransSplat~\cite{zhang2024transplat} & 26.69                                 & 0.875                                 & 0.125                        \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Ablation studies on RealEstate10K.}
        Our method achieves superior performance with half the training steps.
    }
    \label{tab:ablation}
\end{table}

==> ICCV_2025_H3R/tables/camera_norm.tex <==
\begin{table*}[!htbp]
    \centering
    \begin{NiceTabular}{c|ccc|ccc|ccc}
        \CodeBefore
        \rowcolor{heavygray}{3-3}
        \Body

        \toprule
        \textbf{Camera pose}   & \Block{1-3}{\textbf{RealEstate10K}} &                         &                            & \Block{1-3}{\textbf{RealEstate10K $\to$ ACID}} &                         &                            & \Block{1-3}{\textbf{RealEstate10K $\to$ DTU}}                                                        \\
        \textbf{normalization} & \textbf{PSNR$\uparrow$}             & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$}                        & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$}                       & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
        \midrule
        \xmark                 & 27.05                               & 0.882                   & 0.121                      & 28.55                                          & 0.849                   & 0.145                      & \textbf{15.49}                                & \textbf{0.587}          & \textbf{0.314}             \\
        \midrule
        \Block{2-1}{\cmark}    & \textbf{27.08}                      & \textbf{0.883}          & \textbf{0.120}             & \textbf{28.61}                                 & \textbf{0.852}          & \textbf{0.144}             & 15.10                                         & 0.565                   & 0.319                      \\[-3pt]
                               & \diff{+0.03}                        & \diff{+0.001}           & \diff{-0.001}              & \diff{+0.06}                                   & \diff{+0.003}           & \diff{-0.001}              & \diff{-0.39}                                  & \diff{-0.022}           & \diff{+0.005}              \\
        \bottomrule
    \end{NiceTabular}
    \caption{
        \textbf{Effect of camera pose normalization.}
        While camera normalization yields modest improvements on scene-level datasets, it significantly degrades generalization performance on the object-level DTU dataset.
    }
    \label{tab:camera_norm}
\end{table*}

==> ICCV_2025_H3R/tables/cost_function.tex <==
\begin{table}[!tbp]
    \centering
    \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{c|ccc|ccc|ccc}
            \toprule
            \textbf{Cost}     & \multicolumn{3}{c|}{\textbf{RealEstate10K}} & \multicolumn{3}{c|}{\textbf{RealEstate10K $\to$ ACID}} & \multicolumn{3}{c}{\textbf{RealEstate10K $\to$ DTU}}                                                                                                                                                                   \\
            \textbf{Strategy} & \textbf{PSNR$\uparrow$}                     & \textbf{SSIM$\uparrow$}                                & \textbf{LPIPS$\downarrow$}                           & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
            \midrule
            w/o latent volume & 26.56                                       & 0.874                                                  & 0.128                                                & 28.03                   & 0.837                   & 0.157                      & 11.83                   & 0.342                   & 0.540                      \\
            \midrule
            Correlation       & 26.50                                       & 0.872                                                  & 0.129                                                & 28.16                   & 0.842                   & 0.153                      & 15.21                   & 0.567                   & 0.326                      \\
            Difference        & \textbf{26.69}                              & \textbf{0.875}                                         & \textbf{0.126}                                       & \textbf{28.34}          & \textbf{0.844}          & \textbf{0.151}             & 15.36                   & 0.576                   & 0.324                      \\
            \rowcolor{heavygray}
            No cost           & 26.68                                       & \textbf{0.875}                                         & \textbf{0.126}                                       & 28.29                   & \textbf{0.844}          & 0.152                      & \textbf{15.38}          & \textbf{0.587}          & \textbf{0.317}             \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Effect of cost strategies for volumetric latent fusion.}
    }
    \label{tab:cost_function}
\end{table}

==> ICCV_2025_H3R/tables/cross_dataset.tex <==
\begin{table}[!tbp]
    \centering
    \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{l|ccc|ccc|ccc}
            \toprule
            \multirow{2}{*}{\textbf{Method}}         & \multicolumn{3}{c|}{\textbf{ACID}} & \multicolumn{3}{c|}{\textbf{DTU (2 context views)}} & \multicolumn{3}{c}{\textbf{DTU (3 context views)}}                                                                                                                                                                                           \\
                                                     & \textbf{PSNR$\uparrow$}            & \textbf{SSIM$\uparrow$}                             & \textbf{LPIPS$\downarrow$}                         & \textbf{PSNR$\uparrow$}      & \textbf{SSIM$\uparrow$}      & \textbf{LPIPS$\downarrow$}   & \textbf{PSNR$\uparrow$}      & \textbf{SSIM$\uparrow$}      & \textbf{LPIPS$\downarrow$}   \\
            \midrule
            pixelSplat~\cite{charatan2024pixelsplat} & 27.64                              & 0.830                                               & 0.160                                              & 12.89                        & 0.382                        & 0.560                        & 12.52                        & 0.367                        & 0.585                        \\
            MVSplat~\cite{chen2024mvsplat}           & 28.15                              & 0.841                                               & 0.147                                              & 13.94                        & 0.473                        & 0.385                        & 14.30                        & 0.508                        & 0.371                        \\
            TransSplat~\cite{zhang2024transplat}     & 28.17                              & 0.842                                               & 0.146                                              & \cellcolor{tabthird}{14.93}  & 0.531                        & 0.326                        & -                            & -                            & -                            \\
            \midrule
            H3R                                      & \cellcolor{tabthird}{28.79}        & \cellcolor{tabsecond}{0.854}                        & \cellcolor{tabthird}{0.142}                        & \cellcolor{tabsecond}{15.15} & \cellcolor{tabsecond}{0.593} & \cellcolor{tabsecond}{0.305} & \cellcolor{tabthird}{15.27}  & \cellcolor{tabsecond}{0.600} & \cellcolor{tabthird}{0.323}  \\
            H3R-$\alpha$                             & \cellcolor{tabsecond}{28.91}       & \cellcolor{tabsecond}{0.854}                        & \cellcolor{tabsecond}{0.141}                       & \cellcolor{tabfirst}{15.17}  & \cellcolor{tabfirst}{0.605}  & \cellcolor{tabthird}{0.309}  & \cellcolor{tabfirst}{15.98}  & \cellcolor{tabfirst}{0.634}  & \cellcolor{tabfirst}{0.302}  \\
            H3R-$\beta$                              & \cellcolor{tabfirst}{29.23}        & \cellcolor{tabfirst}{0.861}                         & \cellcolor{tabfirst}{0.136}                        & \cellcolor{tabsecond}{15.15} & \cellcolor{tabthird}{0.579}  & \cellcolor{tabfirst}{0.303}  & \cellcolor{tabsecond}{15.36} & \cellcolor{tabthird}{0.599}  & \cellcolor{tabsecond}{0.315} \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Cross-dataset generalization.}
        Models trained on RealEstate10K (indoor) demonstrate strong zero-shot performance on ACID (outdoor) and DTU (object).
    }
    \label{tab:cross_dataset}
    \vspace{-1em}
\end{table}

==> ICCV_2025_H3R/tables/ema.tex <==
\begin{table}[!htbp]
    \centering
    % Use NiceTabular instead of tabular
    \begin{NiceTabular}{c|ccc}
        \CodeBefore
        % Pre-color rows 4–5 to avoid text overlap
        \rowcolor{heavygray}{3-4}
        \Body

        \toprule
        \textbf{EMA}        & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
        \midrule
        \xmark              & 27.42                   & 0.889                   & 0.116                      \\
        \midrule
        % Use \Block instead of \multirow, no longer handles color
        \Block{2-1}{\cmark} & \textbf{27.60}          & \textbf{0.891}          & \textbf{0.114}             \\[-3pt]
                            & \diff{+0.18}            & \diff{+0.002}           & \diff{-0.002}              \\
        \bottomrule
    \end{NiceTabular}
    \caption{
        \textbf{Effect of EMA on RealEstate10K.}
    }
    \label{tab:ema}
\end{table}

==> ICCV_2025_H3R/tables/encoder_performance.tex <==
\begin{table*}[!bp]
    \centering
    \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
            \toprule
            \multirow{2}{*}{\textbf{Encoder}}    & \multirow{2}{*}{\textbf{Res.}} & \multirow{2}{*}{\textbf{Params.}} & \multirow{2}{*}{\textbf{Time (s)$^{\dagger}$}} & \multicolumn{3}{c|}{\textbf{RealEstate10K}} & \multicolumn{3}{c|}{\textbf{RealEstate10K $\rightarrow$ ACID}} & \multicolumn{3}{c|}{\textbf{RealEstate10K $\rightarrow$ DTU}} & \multicolumn{3}{c}{\textbf{Overall}}                                                                                                                                                                                                                                                         \\
                                                 &                                &                                   &                                                & \textbf{PSNR$\uparrow$}                     & \textbf{SSIM$\uparrow$}                                        & \textbf{LPIPS$\downarrow$}                                    & \textbf{PSNR$\uparrow$}              & \textbf{SSIM$\uparrow$}      & \textbf{LPIPS$\downarrow$}   & \textbf{PSNR$\uparrow$}      & \textbf{SSIM$\uparrow$}      & \textbf{LPIPS$\downarrow$}   & \textbf{PSNR$\uparrow$}      & \textbf{SSIM$\uparrow$}      & \textbf{LPIPS$\downarrow$}   \\
            \midrule
            \multicolumn{16}{l}{\color{darkred}{\textbf{\textit{Semantic-aligned}}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
            DeIT III~\cite{touvron2022deit}      & 256                            & \cellcolor{tabthird}{86 M}        & \cellcolor{tabsecond}{0.053}                   & 24.82                                       & 0.832                                                          & 0.156                                                         & 26.26                                & 0.789                        & 0.186                        & 14.44                        & 0.481                        & 0.393                        & 21.84                        & 0.701                        & 0.245                        \\
            CLIP~\cite{radford2021learning}      & 256                            & \cellcolor{tabthird}{86 M}        & \cellcolor{tabfirst}{0.051}                    & 25.14                                       & 0.839                                                          & 0.151                                                         & 26.44                                & 0.791                        & 0.184                        & 14.24                        & 0.475                        & 0.415                        & 21.94                        & 0.702                        & 0.250                        \\
            DINOv2~\cite{oquab2023dinov2}        & 224                            & \cellcolor{tabthird}{86 M}        & \cellcolor{tabfirst}{0.051}                    & 25.74                                       & 0.856                                                          & 0.140                                                         & 26.90                                & 0.809                        & 0.173                        & 14.77                        & 0.502                        & 0.368                        & 22.47                        & 0.722                        & 0.227                        \\
            \midrule
            \multicolumn{16}{l}{\color{darkred}{\textbf{\textit{Spatial-aligned}}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\
            Depth Any.~\cite{yang2024depth}      & 224                            & \cellcolor{tabthird}{86 M}        & 0.056                                          & 26.05                                       & 0.863                                                          & 0.136                                                         & 27.20                                & 0.817                        & 0.168                        & 14.78                        & 0.491                        & 0.368                        & 22.68                        & 0.724                        & 0.224                        \\
            Depth Any. V2~\cite{yang2024depthv2} & 224                            & \cellcolor{tabthird}{86 M}        & \cellcolor{tabthird}{0.054}                    & 25.93                                       & 0.861                                                          & 0.137                                                         & 27.12                                & 0.815                        & 0.169                        & 15.07                        & 0.509                        & 0.360                        & 22.71                        & 0.728                        & 0.222                        \\
            SAM~\cite{kirillov2023segment}       & 256                            & 89 M                              & 0.065                                          & 26.39                                       & 0.869                                                          & \cellcolor{tabthird}{0.130}                                   & 27.79                                & 0.831                        & 0.158                        & 14.95                        & 0.521                        & 0.343                        & 23.04                        & 0.740                        & 0.210                        \\
            SAM 2~\cite{ravi2024sam}             & 256                            & \cellcolor{tabsecond}{68 M}       & \cellcolor{tabthird}{0.054}                    & 26.12                                       & 0.865                                                          & 0.135                                                         & 27.59                                & 0.826                        & 0.163                        & 14.88                        & 0.505                        & 0.361                        & 22.86                        & 0.732                        & 0.220                        \\
            DUSt3R~\cite{wang2024dust3r}         & 256                            & 303 M                             & 0.073                                          & \cellcolor{tabthird}{26.56}                 & \cellcolor{tabthird}{0.873}                                    & \cellcolor{tabsecond}{0.129}                                  & 27.73                                & 0.833                        & 0.158                        & \cellcolor{tabthird}{15.21}  & \cellcolor{tabthird}{0.527}  & \cellcolor{tabthird}{0.342}  & \cellcolor{tabthird}{23.17}  & 0.744                        & 0.210                        \\
            MASt3R~\cite{leroy2025grounding}     & 256                            & 303 M                             & 0.073                                          & \cellcolor{tabsecond}{26.63}                & \cellcolor{tabfirst}{0.876}                                    & \cellcolor{tabfirst}{0.127}                                   & \cellcolor{tabthird}{27.91}          & \cellcolor{tabthird}{0.837}  & \cellcolor{tabthird}{0.156}  & \cellcolor{tabfirst}{15.32}  & \cellcolor{tabsecond}{0.552} & \cellcolor{tabsecond}{0.331} & \cellcolor{tabsecond}{23.29} & \cellcolor{tabsecond}{0.755} & \cellcolor{tabsecond}{0.205} \\
            MAE~\cite{he2022masked}              & 256                            & \cellcolor{tabthird}{86 M}        & \cellcolor{tabfirst}{0.051}                    & \cellcolor{tabfirst}{26.65}                 & \cellcolor{tabsecond}{0.874}                                   & \cellcolor{tabfirst}{0.127}                                   & \cellcolor{tabsecond}{28.04}         & \cellcolor{tabsecond}{0.838} & \cellcolor{tabsecond}{0.154} & \cellcolor{tabsecond}{15.24} & 0.526                        & 0.344                        & \cellcolor{tabfirst}{23.31}  & \cellcolor{tabthird}{0.746}  & \cellcolor{tabthird}{0.208}  \\
            SD-VAE~\cite{rombach2022high}        & 256                            & \cellcolor{tabfirst}{34 M}        & \cellcolor{tabfirst}{0.051}                    & 26.50                                       & 0.872                                                          & \cellcolor{tabsecond}{0.129}                                  & \cellcolor{tabfirst}{28.16}          & \cellcolor{tabfirst}{0.842}  & \cellcolor{tabfirst}{0.153}  & \cellcolor{tabthird}{15.21}  & \cellcolor{tabfirst}{0.567}  & \cellcolor{tabfirst}{0.326}  & \cellcolor{tabsecond}{23.29} & \cellcolor{tabfirst}{0.760}  & \cellcolor{tabfirst}{0.203}  \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Performance comparison across various visual encoders.}
        $^{\dagger}$: Inference time of the entire network.
    }
    \label{tab:encoder_performance}
\end{table*}

==> ICCV_2025_H3R/tables/encoder_type.tex <==
\begin{table}[!bp]
    \centering
    \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{1pt}
        \begin{tabular}{lccc}
            \toprule
            \textbf{Encoder}                     & \textbf{Supervision} & \textbf{Dataset} & \textbf{Arch.}              \\
            \midrule
            \multicolumn{4}{l}{\color{darkred}{\textbf{\textit{Semantic-aligned}}}}                                      \\
            DeIT III~\cite{touvron2022deit}      & Classification       & ImageNet-22k     & ViT-B/16                    \\
            CLIP~\cite{radford2021learning}      & Language             & WIT-400M         & ViT-B/16                    \\
            DINOv2~\cite{oquab2023dinov2}        & Image feature        & LVD-142M         & ViT-B/14                    \\
            \midrule
            \multicolumn{4}{l}{\color{darkred}{\textbf{\textit{Spatial-aligned}}}}                                       \\
            Depth Any.~\cite{yang2024depth}      & Depth                & MIX-14           & ViT-B/14                    \\
            Depth Any. V2~\cite{yang2024depthv2} & Depth                & MIX-13           & ViT-B/14                    \\
            SAM~\cite{kirillov2023segment}       & Segmentation         & SA-1B            & ViT-B/16                    \\
            SAM 2~\cite{ravi2024sam}             & Segmentation         & SA-V             & Hiera~\cite{ryali2023hiera} \\
            DUSt3R~\cite{wang2024dust3r}         & Point regression     & MIX-8            & ViT-L/16                    \\
            MASt3R~\cite{leroy2025grounding}     & Point matching       & MIX-14           & ViT-L/16                    \\
            MAE~\cite{he2022masked}              & Pixel                & ImageNet-1k      & ViT-B/16                    \\
            SD-VAE~\cite{rombach2022high}        & Pixel                & OpenImages       & CNN                         \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Overview of investigated visual foundation models.}
    }
    \label{tab:encoder_type}
\end{table}

==> ICCV_2025_H3R/tables/finetuning.tex <==
\begin{table*}[!htbp]
    \centering
    \begin{NiceTabular}{c|ccc|ccc|ccc}
        \CodeBefore
        \rowcolor{heavygray}{3-3}
        \Body

        \toprule
        \Block{2-1}{\textbf{Finetuning}} & \Block{1-3}{\textbf{RealEstate10K}} &                         &                            & \Block{1-3}{\textbf{RealEstate10K $\to$ ACID}} &                         &                            & \Block{1-3}{\textbf{RealEstate10K $\to$ DTU}}                                                        \\
                                         & \textbf{PSNR$\uparrow$}             & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$}                        & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$}                       & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
        \midrule
        \xmark                           & 26.68                               & 0.875                   & 0.126                      & 28.29                                          & 0.844                   & 0.152                      & 15.38                                         & 0.587                   & 0.317                      \\
        \midrule
        \Block{2-1}{\cmark}              & \textbf{26.81}                      & \textbf{0.878}          & \textbf{0.125}             & \textbf{28.39}                                 & \textbf{0.846}          & \textbf{0.151}             & \textbf{15.63}                                & \textbf{0.598}          & \textbf{0.309}             \\[-3pt]
                                         & \diff{+0.13}                        & \diff{+0.003}           & \diff{-0.001}              & \diff{+0.10}                                   & \diff{+0.002}           & \diff{-0.001}              & \diff{+0.25}                                  & \diff{+0.011}           & \diff{-0.008}              \\
        \bottomrule
    \end{NiceTabular}
    \caption{
        \textbf{Effect of finetuning the SD-VAE encoder.}
    }
    \label{tab:finetuning}
\end{table*}

==> ICCV_2025_H3R/tables/gaussian.tex <==
\begin{table}[!htbp]
    \centering
    \begin{tabular}{c|cc}
        \toprule
        \textbf{Parameter} & \textbf{Activation} & \textbf{Channel} \\
        \midrule
        Center             & None                & 3                \\
        Scale              & Sigmoid             & 3                \\
        Rotation           & L2 norm             & 4                \\
        Opacity            & Sigmoid             & 1                \\
        Color              & ReLU                & 3                \\
        \bottomrule
    \end{tabular}
    \caption{
        \textbf{3D Gaussian parameterization.}
    }
    \label{tab:gaussian}
\end{table}

==> ICCV_2025_H3R/tables/gslrm.tex <==
\begin{table}[!htbp]
    \centering
    \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{3pt}
        \begin{tabular}{c|cc|ccc}
            \toprule
            \multirow{2}{*}{\textbf{Method}} & \textbf{\#Trainable} & \textbf{\#GPU days}  & \multicolumn{3}{c}{\textbf{RealEstate10K}}                                                        \\
                                             & \textbf{Params.}     & \textbf{4090~/~A100} & \textbf{PSNR$\uparrow$}                    & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
            \midrule
            GS-LRM                           & 300M                 & 0~/~192              & \textbf{28.10}                             & 0.892                   & 0.114                      \\
            H3R-$\beta$                      & 91M                  & 30~/~7               & 28.03                                      & \textbf{0.897}          & \textbf{0.110}             \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Comparison with GS-LRM~\cite{zhang2024gs}.}
        We achieve comparable performance with \textbf{30\%} trainable parameters and \textbf{20\%} training cost.
    }
    \label{tab:gslrm}
\end{table}

==> ICCV_2025_H3R/tables/overlap.tex <==
\begin{table*}[!htbp]
    \centering
    \begin{tabular}{c|ccc|ccc|ccc}
        \toprule
        \multirow{2}{*}{\textbf{Overlap}} & \multicolumn{3}{c|}{\textbf{MVSplat}} & \multicolumn{3}{c|}{\textbf{H3R (ours)}} & \multicolumn{3}{c}{\textbf{Improvement}}                                                                                                                                                                                           \\
                                          & \textbf{PSNR$\uparrow$}               & \textbf{SSIM$\uparrow$}                  & \textbf{LPIPS$\downarrow$}               & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{$\Delta$PSNR$\uparrow$} & \textbf{$\Delta$SSIM$\uparrow$} & \textbf{$\Delta$LPIPS$\downarrow$} \\
        \midrule
        $[0.60, 0.65)$                    & 24.41                                 & 0.841                                    & 0.151                                    & 26.14                   & 0.877                   & 0.127                      & +1.73                           & +0.036                          & -0.024                             \\
        $[0.65, 0.70)$                    & 25.00                                 & 0.852                                    & 0.144                                    & 26.44                   & 0.882                   & 0.124                      & +1.44                           & +0.030                          & -0.020                             \\
        $[0.70, 0.75)$                    & 25.68                                 & 0.862                                    & 0.133                                    & 27.00                   & 0.887                   & 0.116                      & +1.32                           & +0.025                          & -0.017                             \\
        $[0.75, 0.80)$                    & 25.74                                 & 0.864                                    & 0.131                                    & 27.01                   & 0.888                   & 0.115                      & +1.27                           & +0.024                          & -0.016                             \\
        $[0.80, 0.85)$                    & 26.15                                 & 0.871                                    & 0.129                                    & 27.33                   & 0.893                   & 0.113                      & +1.18                           & +0.022                          & -0.016                             \\
        $[0.85, 0.90)$                    & 26.18                                 & 0.872                                    & 0.129                                    & 27.39                   & 0.894                   & 0.114                      & +1.21                           & +0.022                          & -0.015                             \\
        $[0.90, 0.95)$                    & 25.92                                 & 0.863                                    & 0.134                                    & 27.12                   & 0.886                   & 0.118                      & +1.20                           & +0.023                          & -0.016                             \\
        $[0.95, 1.00)$                    & 27.86                                 & 0.881                                    & 0.117                                    & 28.93                   & 0.899                   & 0.105                      & +1.07                           & +0.018                          & -0.012                             \\
        \bottomrule
    \end{tabular}
    \caption{
        \textbf{Performance comparison across varying overlaps.}
    }
    \label{tab:overlap}
\end{table*}

==> ICCV_2025_H3R/tables/plucker_latent.tex <==
\begin{table}[!tbp]
    \centering
    \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{cc|ccc|ccc|ccc}
            \toprule
            \textbf{Plücker} & \textbf{Latent} & \multicolumn{3}{c|}{\textbf{RealEstate10K}} & \multicolumn{3}{c|}{\textbf{RealEstate10K $\rightarrow$ ACID}} & \multicolumn{3}{c}{\textbf{RealEstate10K $\rightarrow$ DTU}}                                                                                                                                                                   \\
            \textbf{Coord.}  & \textbf{Volume} & \textbf{PSNR$\uparrow$}                     & \textbf{SSIM$\uparrow$}                                        & \textbf{LPIPS$\downarrow$}                                   & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
            \midrule
            \xmark           & \xmark          & 22.62                                       & 0.754                                                          & 0.205                                                        & 24.11                   & 0.706                   & 0.242                      & 10.42                   & 0.271                   & 0.604                      \\
            \cmark           & \xmark          & 26.56                                       & 0.874                                                          & 0.128                                                        & 28.03                   & 0.837                   & 0.157                      & 11.83                   & 0.342                   & 0.540                      \\
            \xmark           & \cmark          & 26.61                                       & 0.874                                                          & 0.127                                                        & 28.26                   & \textbf{0.844}          & \textbf{0.150}             & \textbf{15.40}          & 0.562                   & 0.324                      \\
            \rowcolor{heavygray}
            \cmark           & \cmark          & \textbf{26.68}                              & \textbf{0.875}                                                 & \textbf{0.126}                                               & \textbf{28.29}          & \textbf{0.844}          & 0.152                      & 15.38                   & \textbf{0.587}          & \textbf{0.317}             \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Effect of Plücker coordinates and latent volume.}
        Best results in \textbf{bold}; our method in \colorbox{heavygray}{gray}.
    }
    \label{tab:plucker_latent}
\end{table}

==> ICCV_2025_H3R/tables/re10k_acid.tex <==
\begin{table}[!htbp]
    \centering
    \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{l|c|ccc|ccc}
            \toprule                                     %
            \multirow{2}{*}{\textbf{Method}}            & \textbf{\#Gaussians}               & \multicolumn{3}{c|}{\textbf{RealEstate10K}~\cite{zhou2018stereo}} & \multicolumn{3}{c}{\textbf{ACID}~\cite{liu2021infinite}}                                                                                                                             \\
                                                        & ($N \times H \times W \times K$)   & \textbf{PSNR$\uparrow$}                                           & \textbf{SSIM$\uparrow$}                                  & \textbf{LPIPS$\downarrow$}   & \textbf{PSNR$\uparrow$}      & \textbf{SSIM$\uparrow$}      & \textbf{LPIPS$\downarrow$}   \\
            \midrule                                     %
            pixelNeRF~\cite{yu2021pixelnerf}            & \multirow{4}{*}{N/A}               & 20.43                                                             & 0.589                                                    & 0.550                        & 20.97                        & 0.547                        & 0.533                        \\
            GPNR~\cite{suhail2022generalizable}         &                                    & 24.11                                                             & 0.793                                                    & 0.255                        & 25.28                        & 0.764                        & 0.332                        \\
            AttnRend~\cite{du2023learning}              &                                    & 24.78                                                             & 0.820                                                    & 0.213                        & 26.88                        & 0.799                        & 0.218                        \\
            MuRF~\cite{xu2024murf}                      &                                    & 26.10                                                             & 0.858                                                    & 0.143                        & 28.09                        & 0.841                        & 0.155                        \\
            \midrule                                     %
            latentSplat~\cite{wewer2025latentsplat}     & $2 \times 256 \times 256 \times 3$ & 23.88                                                             & 0.812                                                    & 0.164                        & -                            & -                            & -                            \\
            pixelSplat~\cite{charatan2024pixelsplat}    & $2 \times 256 \times 256 \times 3$ & 26.09                                                             & 0.863                                                    & 0.136                        & 28.27                        & 0.843                        & 0.146                        \\
            MVSplat~\cite{chen2024mvsplat}              & $2 \times 256 \times 256 \times 1$ & 26.39                                                             & 0.869                                                    & 0.128                        & 28.25                        & 0.843                        & 0.144                        \\
            MVSplat360~\cite{chen2024mvsplat360}        & $2 \times 256 \times 256 \times 1$ & 26.41                                                             & 0.869                                                    & 0.126                        & -                            & -                            & -                            \\
            eFreeSplat~\cite{min2024epipolar}           & $2 \times 256 \times 256 \times 1$ & 26.45                                                             & 0.865                                                    & 0.126                        & 28.30                        & 0.851                        & \cellcolor{tabfirst}{0.140}  \\
            TranSplat~\cite{zhang2024transplat}         & $2 \times 256 \times 256 \times 1$ & 26.69                                                             & 0.875                                                    & 0.125                        & \cellcolor{tabthird}{28.35}  & 0.845                        & 0.143                        \\
            DepthSplat$^{\dag}$~\cite{xu2024depthsplat} & -                                  & 27.44                                                             & \cellcolor{tabthird}{0.887}                              & 0.119                        & -                            & -                            & -                            \\
            \midrule                                     %
            H3R                                         & $2 \times 256 \times 256 \times 1$ & \cellcolor{tabthird}{27.60}                                       & \cellcolor{tabsecond}{0.891}                             & \cellcolor{tabthird}{0.114}  & 28.29                        & \cellcolor{tabthird}{0.846}  & \cellcolor{tabthird}{0.144}  \\
            H3R-$\alpha$                                & $5 \times 256 \times 256 \times 1$ & \cellcolor{tabsecond}{27.79}                                      & \cellcolor{tabsecond}{0.891}                             & \cellcolor{tabsecond}{0.113} & \cellcolor{tabsecond}{28.44} & \cellcolor{tabsecond}{0.847} & \cellcolor{tabthird}{0.144}  \\
            H3R-$\beta$                                 & $2 \times 512 \times 512 \times 1$ & \cellcolor{tabfirst}{28.03}                                       & \cellcolor{tabfirst}{0.897}                              & \cellcolor{tabfirst}{0.110}  & \cellcolor{tabfirst}{28.71}  & \cellcolor{tabfirst}{0.853}  & \cellcolor{tabsecond}{0.141} \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Quantitative evaluation.}
        Each model takes two context images with camera parameters as input and synthesizes three novel views for assessment.
        H3R-$\alpha$ processes multiple context images at 256$\times$256 alongside target-view cameras, while H3R-$\beta$ is optimized for two high-resolution context images at 512$\times$512.
        We highlight the \colorbox{tabfirst}{best}, \colorbox{tabsecond}{second-best}, and \colorbox{tabthird}{third-best} results.
        $^{\dag}$DepthSplat~\cite{xu2024depthsplat} uses additional pre-training data.
    }
    \label{tab:re10k_acid}
\end{table}

==> ICCV_2025_H3R/tables/resolution.tex <==
\begin{table*}[!htbp]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|c|ccc|ccc|ccc}
            \toprule
            \multirow{2}{*}{\textbf{Encoder}}                 & \multirow{2}{*}{\textbf{Res.}} & \multicolumn{3}{c|}{\textbf{RealEstate10K}} & \multicolumn{3}{c|}{\textbf{RealEstate10K $\to$ ACID}} & \multicolumn{3}{c}{\textbf{RealEstate10K $\to$ DTU}}                                                                                                                                                                                     \\
                                                              &                                & \textbf{PSNR$\uparrow$}                     & \textbf{SSIM$\uparrow$}                                & \textbf{LPIPS$\downarrow$}                           & \textbf{PSNR$\uparrow$}     & \textbf{SSIM$\uparrow$}     & \textbf{LPIPS$\downarrow$}  & \textbf{PSNR$\uparrow$}     & \textbf{SSIM$\uparrow$}     & \textbf{LPIPS$\downarrow$}  \\
            \midrule
            DINOv2~\cite{oquab2023dinov2}                     & 224                            & 25.74                                       & 0.856                                                  & 0.140                                                & 26.90                       & 0.809                       & 0.173                       & 14.77                       & 0.502                       & 0.368                       \\
            Depth Any.~\cite{yang2024depth}                   & 224                            & 26.05                                       & 0.863                                                  & 0.136                                                & 27.20                       & 0.817                       & 0.168                       & 14.78                       & 0.491                       & 0.368                       \\
            Depth Any. V2~\cite{yang2024depthv2}              & 224                            & 25.93                                       & 0.861                                                  & 0.137                                                & 27.12                       & 0.815                       & 0.169                       & 15.07                       & 0.509                       & 0.360                       \\
            \midrule
            \multirow{2}{*}{CLIP~\cite{radford2021learning}}  & 224                            & 24.90                                       & 0.832                                                  & 0.155                                                & 26.20                       & 0.782                       & 0.189                       & 13.91                       & 0.448                       & 0.437                       \\
                                                              & 256                            & \cellcolor{tabfirst}{25.14}                 & \cellcolor{tabfirst}{0.839}                            & \cellcolor{tabfirst}{0.151}                          & \cellcolor{tabfirst}{26.44} & \cellcolor{tabfirst}{0.791} & \cellcolor{tabfirst}{0.184} & \cellcolor{tabfirst}{14.24} & \cellcolor{tabfirst}{0.475} & \cellcolor{tabfirst}{0.415} \\
            \midrule
            \multirow{2}{*}{DUSt3R~\cite{wang2024dust3r}}     & 224                            & 26.44                                       & 0.871                                                  & 0.130                                                & 27.63                       & 0.830                       & 0.160                       & \cellcolor{tabfirst}{15.24} & \cellcolor{tabfirst}{0.530} & 0.346                       \\
                                                              & 256                            & \cellcolor{tabfirst}{26.56}                 & \cellcolor{tabfirst}{0.873}                            & \cellcolor{tabfirst}{0.129}                          & \cellcolor{tabfirst}{27.73} & \cellcolor{tabfirst}{0.833} & \cellcolor{tabfirst}{0.158} & 15.21                       & 0.527                       & \cellcolor{tabfirst}{0.342} \\
            \midrule
            \multirow{2}{*}{MASt3R~\cite{leroy2025grounding}} & 224                            & 26.46                                       & 0.872                                                  & 0.130                                                & 27.79                       & 0.834                       & 0.158                       & \cellcolor{tabfirst}{15.32} & 0.541                       & 0.335                       \\
                                                              & 256                            & \cellcolor{tabfirst}{26.63}                 & \cellcolor{tabfirst}{0.876}                            & \cellcolor{tabfirst}{0.127}                          & \cellcolor{tabfirst}{27.91} & \cellcolor{tabfirst}{0.837} & \cellcolor{tabfirst}{0.156} & \cellcolor{tabfirst}{15.32} & \cellcolor{tabfirst}{0.552} & \cellcolor{tabfirst}{0.331} \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Effect of input resolution.}
    }
    \label{tab:resolution}
\end{table*}

==> ICCV_2025_H3R/tables/training_setting_acid.tex <==
\begin{table*}[!htbp]
    \renewcommand{\arraystretch}{1.1} % Adjust row height for readability
    \centering
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{config}      & \textbf{H3R}                                                                 & \textbf{H3R-$\alpha$} & \textbf{H3R-$\beta$} \\
        \midrule
        peak learning rate   & 1e-4                                                                         & 5e-5                  & 5e-5                 \\
        min learning rate    & 5e-5                                                                         & -                     & -                    \\
        warm-up steps        & 3,000                                                                        & 0                     & 0                    \\
        LR schedule          & \begin{tabular}[c]{c}cosine decay\\ 150k steps,\\ then constant\end{tabular} & constant              & constant             \\
        \midrule
        optimizer            & \multicolumn{3}{c}{Adam}                                                                                                    \\
        betas                & \multicolumn{3}{c}{(0.9, 0.999)}                                                                                            \\
        weight decay         & \multicolumn{3}{c}{0}                                                                                                       \\
        gradient clip        & \multicolumn{3}{c}{0.5}                                                                                                     \\
        total batch size     & \multicolumn{3}{c}{16}                                                                                                      \\
        \midrule
        EMA decay            & \multicolumn{3}{c}{0.999}                                                                                                   \\
        \midrule
        trainable parameters & \multicolumn{3}{c}{90.9 M}                                                                                                  \\
        training steps       & 400,000                                                                      & 90,000                & 20,000               \\
        GPU                  & 4 $\times$ RTX 4090                                                          & 8 $\times$ RTX 4090   & 4 $\times$ A100-80GB \\
        training time        & 3 days                                                                       & 28 hours              & 11 hours             \\
        \bottomrule
    \end{tabular}
    \caption{
        \textbf{Training settings for ACID}.
    }
    \label{tab:training_setting_acid}
\end{table*}

==> ICCV_2025_H3R/tables/training_setting_re10k.tex <==
\begin{table*}[!htbp]
    \renewcommand{\arraystretch}{1.1} % Adjust row height for readability
    \centering
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{config}      & \textbf{H3R}                                                                 & \textbf{H3R-$\alpha$} & \textbf{H3R-$\beta$} \\
        \midrule
        peak learning rate   & 1e-4                                                                         & 5e-5                  & 5e-5                 \\
        min learning rate    & 5e-5                                                                         & -                     & -                    \\
        warm-up steps        & 3,000                                                                        & 0                     & 0                    \\
        LR schedule          & \begin{tabular}[c]{c}cosine decay\\ 150k steps,\\ then constant\end{tabular} & constant              & constant             \\
        \midrule
        optimizer            & \multicolumn{3}{c}{Adam}                                                                                                    \\
        betas                & \multicolumn{3}{c}{(0.9, 0.999)}                                                                                            \\
        weight decay         & \multicolumn{3}{c}{0}                                                                                                       \\
        gradient clip        & \multicolumn{3}{c}{0.5}                                                                                                     \\
        total batch size     & \multicolumn{3}{c}{16}                                                                                                      \\
        \midrule
        EMA decay            & \multicolumn{3}{c}{0.999}                                                                                                   \\
        \midrule
        trainable parameters & \multicolumn{3}{c}{90.9 M}                                                                                                  \\
        training steps       & 1,000,000                                                                    & 30,000                & 80,000               \\
        GPU                  & 4 $\times$ RTX 4090                                                          & 4 $\times$ A100-80GB  & 4 $\times$ A100-80GB \\
        training time        & 7.4 days                                                                     & 15 hours              & 42 hours             \\
        \bottomrule
    \end{tabular}
    \caption{
        \textbf{Training settings for RealEstate10K.}
    }
    \label{tab:training_setting_re10k}
\end{table*}

==> ICCV_2025_H3R/tables/view_scaling.tex <==
\begin{table*}[!htbp]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{NiceTabular}{c|ccc|ccc|ccc|ccc}
            \CodeBefore
            \rowcolor{heavygray}{4-5}
            \Body

            \toprule
            \Block{2-1}{\textbf{Method}}     & \multicolumn{3}{c|}{\textbf{RealEstate10K (2 views)}} & \multicolumn{3}{c|}{\textbf{RealEstate10K (4 views)}} & \multicolumn{3}{c|}{\textbf{RealEstate10K (6 views)}} & \multicolumn{3}{c}{\textbf{RealEstate10K (8 views)}}                                                                                                                                                                                                                          \\
                                             & \textbf{PSNR$\uparrow$}                               & \textbf{SSIM$\uparrow$}                               & \textbf{LPIPS$\downarrow$}                            & \textbf{PSNR$\uparrow$}                              & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
            \midrule
            MVSplat                          & 26.36                                                 & 0.868                                                 & 0.129                                                 & 22.20                                                & 0.820                   & 0.118                      & 20.95                   & 0.803                   & 0.203                      & 20.35                   & 0.792                   & 0.214                      \\
            \midrule
            \Block{2-1}{H3R-$\alpha$ (Ours)} & \textbf{27.46}                                        & \textbf{0.889}                                        & \textbf{0.115}                                        & \textbf{29.28}                                       & \textbf{0.920}          & \textbf{0.090}             & \textbf{29.97}          & \textbf{0.930}          & \textbf{0.083}             & \textbf{30.24}          & \textbf{0.934}          & \textbf{0.080}             \\[-3pt]
                                             & \diff{+1.10}                                          & \diff{+0.021}                                         & \diff{-0.014}                                         & \diff{+7.08}                                         & \diff{+0.100}           & \diff{-0.028}              & \diff{+9.02}            & \diff{+0.127}           & \diff{-0.120}              & \diff{+9.89}            & \diff{+0.142}           & \diff{-0.134}              \\
            \bottomrule
        \end{NiceTabular}
    }
    \caption{
        \textbf{Performance comparison across varying number of input views.}
    }
    \label{tab:view_scaling}
\end{table*}
